Context-Aware Assistant Selection for Improved Inference Acceleration with Large Language Models

Despite their widespread adoption, large language models (LLMs) remain prohibitive to use under resource constraints, with their ever growing sizes only increasing the barrier for use. One noted issue is the high latency associated with auto-regressive generation, rendering large LLMs use dependent on advanced computing infrastructure. Assisted decoding, where a smaller draft model guides a larger target model's generation, has helped alleviate this, but remains dependent on alignment between the two models. Thus if the draft model is insufficiently capable on some domain relative to the target model, performance can degrade. Alternatively, one can leverage multiple draft models to better cover the expertise of the target, but when multiple black-box draft models are available, selecting an assistant without details about its construction can be difficult. To better understand this decision making problem, we observe it as a contextual bandit, where a policy must choose a draft model based on a context. We show that even without prior knowledge of the draft models, creating an offline dataset from only outputs of independent draft/target models and training a policy over the alignment of these outputs can accelerate performance on multiple domains provided the candidates are effective. Further results show this to hold on various settings with multiple assisted decoding candidates, highlighting its flexibility and the advantageous role that such decision making can play.

==> objects/gsm8k.tex <==
% \begin{table}[ht!]
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{l|cc}
%         \toprule
%         \textsc{Draft Candidate} & \textbf{\textsc{Rouge-L}} & \textbf{Decoding Speed} \\
%         \midrule
%         Auto-Regressive & $21.47$ & $1.00\times$ (22.03 ms/token) \\
%         \texttt{T5-Small} & $20.91$ & $0.78\times$ (28.08 ms/token) \\
%         \texttt{T5-Small-XSum} & $20.24$ & $0.74\times$ (29.91 ms/token) \\
%         \midrule
%         Greedy $\pi_\theta$ & $21.21$ & $0.98\times$ (22.54 ms/token) \\
%         Dynamic $\pi_\theta$ & $21.20$ & $0.98\times$ (22.45 ms/token) \\
%         \bottomrule
%         \end{tabular}
%     }
%     \caption{Decoding speeds on \textsc{GSM8K} with a \texttt{Flan-T5-XXL} expert. Policies are trained on all three tasks (\textsc{GSM8K}, \textsc{XSum}, \textsc{En-De}). Inference on the latter two tasks is negligibly different from \autoref{tab:with_autoregressive}.}
%     \label{tab:gsm8k}
% \end{table}

\begin{table}[ht!]
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cc}
        \toprule
        \textsc{Draft Candidate} & \textbf{\textsc{Accuracy}} & \textbf{Decoding Speed} \\
        \midrule
        Auto-Regressive & $10.67$ & $1.00\times$ (22.03 ms/token) \\
        \texttt{T5-Small} & $10.99$ & $0.78\times$ (28.08 ms/token) \\
        \texttt{T5-Small-XSum} & $10.09$ & $0.74\times$ (29.91 ms/token) \\
        \midrule
        Greedy $\pi_\theta$ & $10.64$ & $0.95\times$ (23.54 ms/token) \\
        Dynamic $\pi_\theta$ & $10.38$ & $0.95\times$ (23.45 ms/token) \\
        \bottomrule
        \end{tabular}
    }
    \caption{Decoding speeds on \textsc{GSM8K} (test set) with a \texttt{Flan-T5-XXL} expert. 
    % Policies are trained on all three tasks (\textsc{GSM8K}, \textsc{XSum}, \textsc{En-De}).
    Inference on the latter two tasks is negligibly different from \autoref{tab:with_autoregressive}.}
    \label{tab:gsm8k}
\end{table}

==> objects/sorted-ood.tex <==
\paragraph{Generalizing to OOD Contexts.}
% \begin{table}[ht!]
\begin{wraptable}{r}{0.4\linewidth}
    \resizebox{\linewidth}{!}{
        \centering
        \begin{tabular}{l|cc}
        \toprule
        \textsc{Strategy} & \textsc{Self-Instruct} \\
        \midrule
        \multicolumn{2}{c}{\textbf{IndepEn-Dent}} \\
        \midrule
        Auto-regressive & \\
        \midrule
        \multicolumn{2}{c}{\textbf{Intermediate Drafting}} \\
        \midrule
        Layer 8 Drafting & \\
        Layer 16 Drafting & \\
        Layer 24 Drafting & \\
        Layer 32 Drafting & \\
        \midrule
        \multicolumn{2}{c}{\textbf{Intermediate Drafting + Policy}} \\
        \midrule
        Greedy Policy $\pi_\theta$ & \\
        Dynamic Policy $\pi_\theta$ & \\
        \bottomrule
        \end{tabular}
    }
    \caption{
        Performance on on a out-of-distribution testing dataset (\textsc{Self-Instruct}) using a \texttt{LLaMA-2-13B-Chat} model fine-tuned on \textsc{Alpaca} following~\citep{kavehzadeh2024sorted}.
    }
    \label{tab:sorted-ood}
% \end{table}
\end{wraptable}
